OpenMaterial: A Large-scale Dataset of Complex Materials for 3D Reconstruction

Recent advances in deep learning, such as neural radiance fields and implicit neural representations, have significantly advanced 3D reconstruction. However, accurately reconstructing objects with complex optical properties, such as metals, glass, and plastics, remains challenging due to the breakdown of multi-view color consistency in the presence of specular reflections, refractions, and transparency. This limitation is further exacerbated by the lack of benchmark datasets that explicitly model material-dependent light transport. To address this, we introduce OpenMaterial, a large-scale semi-synthetic dataset for benchmarking material-aware 3D reconstruction. It comprises 1,001 objects spanning 295 distinct materials, including conductors, dielectrics, plastics, and their roughened variants, captured under 714 diverse lighting conditions. By integrating lab-measured Index of Refraction (IOR) spectra, OpenMaterial enables the generation of high-fidelity multi-view images that accurately simulate complex light-matter interactions. It provides multi-view images, 3D shape models, camera poses, depth maps, and object masks, establishing the first extensive benchmark for evaluating 3D reconstruction on challenging materials. We evaluate 11 state-of-the-art methods for 3D reconstruction and novel view synthesis, conducting ablation studies to assess the impact of material type, shape complexity, and illumination on reconstruction performance. Our results indicate that OpenMaterial provides a strong and fair basis for developing more robust, physically-informed 3D reconstruction techniques to better handle real-world optical complexities.

==> fig/ablation-preview/preview1.tex <==
\begin{figure*}[htp]
    \setlength{\belowcaptionskip}{-5pt}
    \renewcommand{\arraystretch}{0.2}
    \setlength{\tabcolsep}{10pt}
    \vspace{-0.5cm}
    \hspace{1.cm}
    
    \begin{minipage}{\textwidth}
    \begin{tabular}{cccc}
    \centering
        & Indoor Scene & Daytime Garden  & Nighttime Street  \\ % \hline
    % \vspace{-5pt} \\
    \rotatebox{90}{\parbox{\imghe}{\centering Conductor}} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_conductor_leadenhall_market_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_conductor_symmetrical_garden_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_conductor_cobblestone_street_night_4k_12.png} \\
    
    \rotatebox{90}{\parbox{\imghe}{\centering RoughConductor}} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_roughconductor_leadenhall_market_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_roughconductor_symmetrical_garden_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_roughconductor_cobblestone_street_night_4k_12.png} \\
    
    \rotatebox{90}{\parbox{\imghe}{\centering Dielectric}} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_dielectric_leadenhall_market_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_dielectric_symmetrical_garden_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_dielectric_cobblestone_street_night_4k_12.png} \\
    
    \rotatebox{90}{\parbox{\imghe}{\centering RoughDielectric}} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_roughdielectric_leadenhall_market_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_roughdielectric_symmetrical_garden_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_roughdielectric_cobblestone_street_night_4k_12.png} \\
    
    \rotatebox{90}{\parbox{\imghe}{\centering Plastic}} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_plastic_leadenhall_market_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_plastic_symmetrical_garden_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_plastic_cobblestone_street_night_4k_12.png} \\
    
    \rotatebox{90}{\parbox{\imghe}{\centering RoughPlastic}} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_roughplastic_leadenhall_market_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_roughplastic_symmetrical_garden_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_roughplastic_cobblestone_street_night_4k_12.png} \\
    
    \rotatebox{90}{\parbox{\imghe}{\centering Diffuse}} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_diffuse_leadenhall_market_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_diffuse_symmetrical_garden_4k_12.png} &
    \includegraphics[width=.24\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_diffuse_cobblestone_street_night_4k_12.png} \\
    
    \end{tabular}
    \end{minipage}
    \caption{\textbf{Previews of the 'Vase' in the ablation dataset.}}
    \label{fig:ablation_preview-1}
\end{figure*}


==> fig/camera_poses.tex <==
\begin{wrapfigure}[12]{r}{0.4\linewidth}
    \centering
    \includegraphics[width=0.964\linewidth]{img/camera_poses.png}
    \caption{Camera positions \ZD{Might need to refine} \HJL{Can this picture be deleted?}}
    \label{fig:cameras}
\end{wrapfigure}

==> fig/dataset-comparison-selected.tex <==
\begin{figure*}[htb]
\setlength{\belowcaptionskip}{-10pt}
\centering
\includegraphics[height=0.17\textwidth]{img/datasets/ShinyBlender(ref-nerf)/6.png}
\hspace{.5cm}
\includegraphics[height=0.17\textwidth]{img/datasets/ref_nerf_real/3.jpg}
\hspace{.3cm}
\includegraphics[height=0.17\textwidth]{img/Chicago_Bean.jpeg}
\hspace{.3cm}
\includegraphics[height=0.17\textwidth]{img/datasets/openmaterial/Conductor/fc4f34dae22c4dae95c19b1654c3cb7e/conductor-Lu/033.png}
% \includegraphics[height=0.19\textwidth]{img/ablation_preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/leadenhall_market_4k-conductor.png}
\caption{\label{fig:dataset-comp-selected} \textbf{Data comparison.} From left to right ShinyBlender, Ref-Nerf (Real), Chicago Bean (Web image), Ours.}
\end{figure*}


==> fig/dataset-comparison.tex <==
\begin{figure*}[htb]
    % \setlength{\belowcaptionskip}{-10pt}
    \centering
    \renewcommand{\arraystretch}{1.0}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{cccccc}
        \includegraphics[width=0.16\textwidth]{img/datasets/select/1-1.png} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/1-2.png} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/1-3.png} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/1-4.png} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/1-5.png} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/1-6.png} \\
        
        \includegraphics[width=0.16\textwidth]{img/datasets/select/2-1.jpg} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/2-2.jpg} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/2-3.jpg} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/2-4.jpg} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/2-5.png} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/2-6.png} \\

        \includegraphics[width=0.16\textwidth]{img/datasets/select/3-1.jpg} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/3-2.jpg} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/3-3.jpg} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/3-4.png} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/3-5.png} &
        \includegraphics[width=0.16\textwidth]{img/datasets/select/3-6.png} \\
    \end{tabular}
    \caption{\label{fig:dataset-comparison} \textbf{Full dataset comparison.} Top row: our dataset, Second row: other datasets with background, third row: other datasets without background}
\end{figure*}




==> fig/nerf_full.tex <==
\newcommand{\imgwidth}{.132\textwidth}
\newcommand{\imgheight}{0.09\textwidth}
\newcommand{\textsize}[1]{{\tiny{#1}}}
\begin{figure}[htp]
    \centering
    \renewcommand{\arraystretch}{0.65}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{ccccc}
    & \raisebox{-2.0ex}{\textsize{Diffuse}} & \raisebox{-2.0ex}{\textsize{Plastic}}  & \raisebox{-2.0ex}{\textsize{Dielectric}} &  \raisebox{-2.0ex}{\textsize{Conductor}}  \\
    % & \raisebox{-2.0ex}{\textsize{Diffuse}} & \raisebox{-2.0ex}{\textsize{Plastic}} & \raisebox{-2.0ex}{\textsize{RoughPlastic}} & \raisebox{-2.0ex}{\textsize{Dielectric}} & \raisebox{-2.0ex}{\textsize{RoughDielectric}} & \raisebox{-2.0ex}{\textsize{Conductor}} & \raisebox{-2.0ex}{\textsize{RoughConductor}} \\

    \rotatebox{90}{\parbox{\imgheight}{\centering \textsize{Groundtruth}}} &
    \includegraphics[width=\imgwidth]{img/vis-nerf/2d_gt_diffuse.jpg} & % name should be 2d_gt_XXXX.png
    \includegraphics[width=\imgwidth]{img/vis-nerf/2d_gt_plastic.jpg} &
    % \includegraphics[width=\imgwidth]{img/vis-nerf/2d_gt_roughplastic.jpg} &
    \includegraphics[width=\imgwidth]{img/vis-nerf/2d_gt_dielectric.jpg} &
    % \includegraphics[width=\imgwidth]{img/vis-nerf/2d_gt_roughdielectric.jpg} &
    \includegraphics[width=\imgwidth]{img/vis-nerf/2d_gt_conductor.jpg} &
    % \includegraphics[width=\imgwidth]{img/vis-nerf/2d_gt_roughconductor.jpg} \\

    \rotatebox{90}{\parbox{\imgheight}{\centering \textsize{method1}}} &
    \includegraphics[width=\imgwidth]{img/vis-nerf/gaussian_diffuse.jpg} & % name should be gaussian_XXXX.png
    \includegraphics[width=\imgwidth]{img/vis-nerf/gaussian_plastic.jpg} &
    % \includegraphics[width=\imgwidth]{img/vis-nerf/gaussian_roughplastic.jpg} &
    \includegraphics[width=\imgwidth]{img/vis-nerf/gaussian_dielectric.jpg} &
    % \includegraphics[width=\imgwidth]{img/vis-nerf/gaussian_roughdielectric.jpg} &
    \includegraphics[width=\imgwidth]{img/vis-nerf/gaussian_conductor.jpg} &
    % \includegraphics[width=\imgwidth]{img/vis-nerf/gaussian_roughconductor.jpg} \\

    \rotatebox{90}{\parbox{\imgheight}{\centering \textsize{method2}}} &
    \includegraphics[width=\imgwidth]{img/vis-nerf/ngp_diffuse.jpg} & % name should be ngp_XXXX.png
    \includegraphics[width=\imgwidth]{img/vis-nerf/ngp_plastic.jpg} &
    % \includegraphics[width=\imgwidth]{img/vis-nerf/ngp_roughplastic.jpg} &
    \includegraphics[width=\imgwidth]{img/vis-nerf/ngp_dielectric.jpg} &
    % \includegraphics[width=\imgwidth]{img/vis-nerf/ngp_roughdielectric.jpg} &
    \includegraphics[width=\imgwidth]{img/vis-nerf/ngp_conductor.jpg} &
    % \includegraphics[width=\imgwidth]{img/vis-nerf/2d_gt_roughconductor.jpg} \\
    \end{tabular}
\caption{\label{fig:nerf} Qualitative result on the novel view synthesis task, top is gt, middle is gaussian splatting, bottom is instant-ngp}
\end{figure}


==> fig/novel_view_synthesis-a.tex <==
\begin{figure*}[htb]
    \setlength{\tabcolsep}{1.25pt}
    \setlength{\belowcaptionskip}{-20pt}
    \renewcommand{\arraystretch}{0.5}
    \begin{minipage}{\textwidth}
    % Start of centering for all tables
    \begin{tabular}{cc}
    \hspace{1.1cm}
        % Left big image
        \begin{minipage}{.40\textwidth}
            \includegraphics[width=\textwidth]{img/vis-nerf-sub/2d_gt_conductor.png}
        \end{minipage} &
        % Right small images in 2x3 grid
        \begin{minipage}{.148\textwidth}
            \begin{tabular}{ccc}
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/gt-conductor.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/PGSR-conductor.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/ngp-conductor.png} \\
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/gt-conductor-1.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/PGSR-conductor-1.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/ngp-conductor-1.png} \\
            \end{tabular}
        \end{minipage}
    \end{tabular}

    \begin{tabular}{cc}
    \hspace{1.1cm}
        % Left big image
        \begin{minipage}{.40\textwidth}
            \includegraphics[width=\textwidth]{img/vis-nerf-sub/2d_gt_dielectric.png}
        \end{minipage} &
        
        % Right small images in 2x3 grid
        \begin{minipage}{.148\textwidth}
            \begin{tabular}{ccc}
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/gt-dielectric.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/PGSR-dielectric.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/ngp-dielectric.png} \\
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/gt-dielectric-1.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/PGSR-dielectric-1.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/ngp-dielectric-1.png} \\
            \end{tabular}
        \end{minipage}
    \end{tabular}

    \begin{tabular}{cc}
    \hspace{1.1cm}
        % Left big image
        \begin{minipage}{.40\textwidth}
            \includegraphics[width=\textwidth]{img/vis-nerf-sub/2d_gt_plastic.png}
        \end{minipage} &
        
        % Right small images in 2x3 grid
        \begin{minipage}{.148\textwidth}
            \begin{tabular}{ccc}
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/gt-plastic.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/PGSR-plastic.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/ngp-plastic.png} \\
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/gt-plastic-1.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/PGSR-plastic-1.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/ngp-plastic-1.png} \\
            \end{tabular}
        \end{minipage}
    \end{tabular}

    \begin{tabular}{cc}
    \hspace{1.1cm}
        % Left big image
        \begin{minipage}{.40\textwidth}
            \includegraphics[width=\textwidth]{img/vis-nerf-sub/2d_gt_diffuse.png}
        \end{minipage} &
        
        % Right small images in 2x3 grid
        \begin{minipage}{.148\textwidth}
            \begin{tabular}{ccc}
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/gt-diffuse.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/PGSR-diffuse.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/ngp-diffuse.png} \\
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/gt-diffuse-1.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/PGSR-diffuse-1.png} &
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/ngp-diffuse-1.png} \\
            \end{tabular}
        \end{minipage}
    \end{tabular}
    \end{minipage}
    \caption{\label{fig:nerf_appendix} \textbf{Qualitative result on the novel view synthesis task.} From top to bottom: Conductor, Dielectric, Plastic, Diffuse. From left to right: GT (global), GT (local), PGSR, Instant-NGP.}
\end{figure*}


==> fig/novel_view_synthesis-ablation-1.tex <==
\begin{figure*}[htp]
    \setlength{\belowcaptionskip}{-.5cm}
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt}
    \begin{minipage}{\textwidth}
    \begin{tabular}{ccccc}
        & Conductor & Dielectric  & Plastic & Diffuse  \\ % \hline
        \vspace{-5pt} \\
        \rotatebox{90}{\parbox{\imghe}{\centering Ground Truth}} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_dielectric_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_plastic_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_diffuse_leadenhall_market_4k_12.png} \\
        
        \rotatebox{90}{\parbox{\imghe}{\centering 3DGS}} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gaussian_model_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gaussian_model_dielectric_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gaussian_model_plastic_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gaussian_model_diffuse_leadenhall_market_4k_12.png} \\

        \rotatebox{90}{\parbox{\imghe}{\centering Instant-NGP}} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/insr_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/insr_dielectric_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/insr_plastic_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/insr_diffuse_leadenhall_market_4k_12.png} \\
        
        \rotatebox{90}{\parbox{\imghe}{\centering PGSR}} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/PGSR_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/PGSR_dielectric_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/PGSR_plastic_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/PGSR_diffuse_leadenhall_market_4k_12.png} \\

        \rotatebox{90}{\parbox{\imghe}{\centering 2DGS}} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/2dgs_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/2dgs_dielectric_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/2dgs_plastic_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/2dgs_diffuse_leadenhall_market_4k_12.png} \\

        \rotatebox{90}{\parbox{\imghe}{\centering GaussianShader}} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/GaussianShader_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/GaussianShader_dielectric_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/GaussianShader_plastic_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/GaussianShader_diffuse_leadenhall_market_4k_12.png} \\

        
        \rotatebox{90}{\parbox{\imghe}{\centering GES}} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/ges_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/ges_dielectric_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/ges_plastic_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/ges_diffuse_leadenhall_market_4k_12.png} \\
        
        \rotatebox{90}{\parbox{\imghe}{\centering GSDR}} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gsdr_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gsdr_dielectric_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gsdr_plastic_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gsdr_diffuse_leadenhall_market_4k_12.png} \\
        
    \end{tabular}
    \caption{\label{fig:nerf_appendix-ablation-1} \textbf{Additional qualitative 3D reconstruction results on the ablation dataset.}}
    \end{minipage}
\end{figure*}

==> fig/novel_view_synthesis-ablation-2.tex <==
\begin{figure*}[htp]
    \setlength{\belowcaptionskip}{-.5cm}
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt}
    \begin{minipage}{\textwidth}
    \begin{tabular}{ccccc}
        & Conductor & Dielectric  & Plastic & Diffuse  \\ % \hline
        \vspace{-5pt} \\
        \rotatebox{90}{\parbox{\imghe}{\centering Ground Truth}} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_dielectric_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_plastic_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_diffuse_leadenhall_market_4k_12.png} \\
        
        \rotatebox{90}{\parbox{\imghe}{\centering GaussianShader}} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/GaussianShader_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/GaussianShader_dielectric_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/GaussianShader_plastic_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/GaussianShader_diffuse_leadenhall_market_4k_12.png} \\

        
        \rotatebox{90}{\parbox{\imghe}{\centering GES}} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/ges_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/ges_dielectric_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/ges_plastic_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/ges_diffuse_leadenhall_market_4k_12.png} \\
        
        \rotatebox{90}{\parbox{\imghe}{\centering GSDR}} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gsdr_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gsdr_dielectric_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gsdr_plastic_leadenhall_market_4k_12.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_nerf/b14a251fe8ad4a10bbc75f7dd3f6cebb/gsdr_diffuse_leadenhall_market_4k_12.png} \\

        
        
    \end{tabular}
    \caption{\label{fig:nerf_appendix-ablation-2} \textbf{Additional qualitative 3D reconstruction results on the ablation dataset (Part 2 of 2).}}
    \end{minipage}
\end{figure*}

==> fig/novel_view_synthesis_2.tex <==
\newcommand{\bigimgwidth}{.25\textwidth}
\newcommand{\smallimgwidth}{.1\textwidth}
\begin{figure*}[t]
    \setlength{\tabcolsep}{1.25pt}
    \renewcommand{\arraystretch}{0.5}
    \begin{tabular}{cccc}
        % Left big image
        \begin{minipage}{\bigimgwidth}
            \includegraphics[width=\textwidth]{img/vis-nerf-sub/2d_gt_conductor.png}
            \raisebox{2pt}[0pt][0pt]{\makebox[\textwidth][c]{Conductor}}
        \end{minipage} &
        \hspace{7pt}
        % Right small images in 2x3 grid
        \begin{minipage}{\smallimgwidth}
            \centering
            \begin{tabular}{cc}
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/PGSR-conductor.png} &
                \hspace{5pt}
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/ngp-conductor.png} \\
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/PGSR-conductor-1.png} &
                \hspace{5pt}
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/ngp-conductor-1.png} \\
                \multicolumn{1}{c}{PGSR~\cite{Chen24}} & \multicolumn{1}{c}{InstantNGP~\cite{Muller22}}
            \end{tabular}
        \end{minipage}

        % Left big image
        \begin{minipage}{\bigimgwidth}
            \includegraphics[width=\textwidth]{img/vis-nerf-sub/2d_gt_dielectric.png}
            \raisebox{2pt}[0pt][0pt]{\makebox[\textwidth][c]{Dielectric}}
        \end{minipage} &
        \hspace{7pt}
        % Right small images in 2x3 grid
        \begin{minipage}{\smallimgwidth}
            \centering
            \begin{tabular}{cc}
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/PGSR-dielectric.png} &
                \hspace{5pt}
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/ngp-dielectric.png} \\
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/PGSR-dielectric-1.png} &
                \hspace{5pt}
                \includegraphics[width=\textwidth]{img/vis-nerf-sub/ngp-dielectric-1.png} \\
                \multicolumn{1}{c}{PGSR~\cite{Chen24}} & \multicolumn{1}{c}{InstantNGP~\cite{Muller22}}
            \end{tabular}
            \raisebox{2pt}[0pt][0pt]{\makebox[\textwidth][c]{ }}
        \end{minipage}
    \end{tabular}

\caption{\label{fig:nerf} \textbf{Qualitative results for novel view synthesis.} From left to right: GT (global), GT (local), PGSR, Instant-NGP}
\end{figure*}


==> fig/physics.tex <==
\begin{figure*}[htp]
    \centering
    % \setlength{\belowcaptionskip}{-10pt}
    \renewcommand{\arraystretch}{0.65}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{cccc}
        \includegraphics[width=.32\textwidth]{img/physics/Conductor.png} &
        \includegraphics[width=.32\textwidth]{img/physics/Dielectric.png} &
        \includegraphics[width=.32\textwidth]{img/physics/Plastic.png} 
        % & \includegraphics[width=.24\textwidth]{img/physics/Diffuse.png} 
        \\
        \includegraphics[width=.32\textwidth]{img/physics/Rough-Conductor.png} &
        \includegraphics[width=.32\textwidth]{img/physics/Rough-Dielectric.png} &
        \includegraphics[width=.32\textwidth]{img/physics/Rough-Plastic.png} &
        
    \end{tabular}
    \caption{\label{fig:physics_full} \textbf{Illustration of light interaction with various materials.}}
\end{figure*}


==> fig/physics_selected.tex <==
\begin{figure}[htp]
    \centering
    \setlength{\belowcaptionskip}{-10pt}
    \renewcommand{\arraystretch}{0.65}
    \setlength{\tabcolsep}{-4pt}
    \begin{tabular}{cccc}
        \includegraphics[width=.36\linewidth]{img/physics/Conductor.png} &
        \includegraphics[width=.36\linewidth]{img/physics/Dielectric.png} &
        \includegraphics[width=.36\linewidth]{img/physics/Plastic.png} 
    \end{tabular}
    \caption{\label{fig:physics} \textbf{Illustration of light interaction with various materials.}}
\end{figure}


==> fig/reconstruction-a-1.tex <==

\begin{figure*}[htb]
    \setlength{\belowcaptionskip}{-.5cm}
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt}
    \begin{minipage}{\textwidth}
    \begin{tabular}{ccccc}
        & Conductor & Dielectric  & Plastic & Diffuse  \\ % \hline
        \vspace{-5pt} \\
        \rotatebox{90}{\parbox{\imghe}{\centering RGB Image}} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_df894b66e2e54b558a43497becb94ff0-conductor.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_a2210a0ba6834141af3bf83ee1e03f07-dielectric.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_ff7e50857e0140f99f1885f3d2c9e4d3-plastic.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_7f350ea007a8462abe573f870a432679-diffuse.png} \\
        
        \rotatebox{90}{\parbox{\imghe}{\centering Ground Truth}} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_df894b66e2e54b558a43497becb94ff0_11.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_a2210a0ba6834141af3bf83ee1e03f07_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_ff7e50857e0140f99f1885f3d2c9e4d3_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_7f350ea007a8462abe573f870a432679_10.png} \\
        
        \rotatebox{90}{\parbox{\imghe}{\centering PGSR}} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/PGSR_df894b66e2e54b558a43497becb94ff0_11.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/PGSR_a2210a0ba6834141af3bf83ee1e03f07_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/PGSR_ff7e50857e0140f99f1885f3d2c9e4d3_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/PGSR_7f350ea007a8462abe573f870a432679_10.png} \\
        
        \rotatebox{90}{\parbox{\imghe}{\centering 2DGS}} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/2dgs_df894b66e2e54b558a43497becb94ff0_11.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/2dgs_a2210a0ba6834141af3bf83ee1e03f07_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/2dgs_ff7e50857e0140f99f1885f3d2c9e4d3_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/2dgs_7f350ea007a8462abe573f870a432679_10.png} \\

        \rotatebox{90}{\parbox{\imghe}{\centering NeRRF}} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/nerrf_df894b66e2e54b558a43497becb94ff0_11.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/nerrf_a2210a0ba6834141af3bf83ee1e03f07_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/nerrf_ff7e50857e0140f99f1885f3d2c9e4d3_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/nerrf_7f350ea007a8462abe573f870a432679_10.png} \\

        \rotatebox{90}{\parbox{\imghe}{\centering NeRO}} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/NeRO_df894b66e2e54b558a43497becb94ff0_11.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/NeRO_a2210a0ba6834141af3bf83ee1e03f07_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/NeRO_ff7e50857e0140f99f1885f3d2c9e4d3_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/NeRO_7f350ea007a8462abe573f870a432679_10.png} \\

        \rotatebox{90}{\parbox{\imghe}{\centering Instant-NGP}} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/instant-nsr-pl-wmask_df894b66e2e54b558a43497becb94ff0_11.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/instant-nsr-pl-wmask_a2210a0ba6834141af3bf83ee1e03f07_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/instant-nsr-pl-wmask_ff7e50857e0140f99f1885f3d2c9e4d3_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/instant-nsr-pl-wmask_7f350ea007a8462abe573f870a432679_10.png} \\

        \rotatebox{90}{\parbox{\imghe}{\centering NeuS2}} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/neus2_df894b66e2e54b558a43497becb94ff0_11.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/neus2_a2210a0ba6834141af3bf83ee1e03f07_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/neus2_ff7e50857e0140f99f1885f3d2c9e4d3_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/neus2_7f350ea007a8462abe573f870a432679_10.png} \\
    \end{tabular}
    \caption{\label{fig:neus_appendix-1} \textbf{Additional qualitative 3D reconstruction results on OpenMaterial.}}
    \end{minipage}
\end{figure*}

==> fig/reconstruction-a-2.tex <==
\begin{figure*}[htp]
    \setlength{\belowcaptionskip}{-.5cm}
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt}
    \begin{minipage}{\textwidth}
    \begin{tabular}{ccccc}
        & Conductor & Dielectric  & Plastic & Diffuse  \\ % \hline
        \vspace{-5pt} \\
        \rotatebox{90}{\parbox{\imghe}{\centering RGB Image}} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_df894b66e2e54b558a43497becb94ff0-conductor.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_a2210a0ba6834141af3bf83ee1e03f07-dielectric.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_ff7e50857e0140f99f1885f3d2c9e4d3-plastic.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_7f350ea007a8462abe573f870a432679-diffuse.png} \\
        
        \rotatebox{90}{\parbox{\imghe}{\centering Ground Truth}} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_df894b66e2e54b558a43497becb94ff0_11.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_a2210a0ba6834141af3bf83ee1e03f07_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_ff7e50857e0140f99f1885f3d2c9e4d3_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_7f350ea007a8462abe573f870a432679_10.png} \\

        \rotatebox{90}{\parbox{\imghe}{\centering Instant-NGP}} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/instant-nsr-pl-wmask_df894b66e2e54b558a43497becb94ff0_11.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/instant-nsr-pl-wmask_a2210a0ba6834141af3bf83ee1e03f07_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/instant-nsr-pl-wmask_ff7e50857e0140f99f1885f3d2c9e4d3_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/instant-nsr-pl-wmask_7f350ea007a8462abe573f870a432679_10.png} \\

        \rotatebox{90}{\parbox{\imghe}{\centering NeuS2}} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/neus2_df894b66e2e54b558a43497becb94ff0_11.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/neus2_a2210a0ba6834141af3bf83ee1e03f07_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/neus2_ff7e50857e0140f99f1885f3d2c9e4d3_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/neus2_7f350ea007a8462abe573f870a432679_10.png} \\
    \end{tabular}
    \caption{\label{fig:neus_appendix-2} \textbf{Additional qualitative 3D reconstruction results on OpenMaterial (Part 2 of 2).}}
    \end{minipage}
\end{figure*}

==> fig/reconstruction-ablation.tex <==
\begin{figure*}[htp]
    \setlength{\belowcaptionskip}{-.5cm}
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt}
    \begin{minipage}{\textwidth}
    \begin{tabular}{ccccc}
        & Conductor & Dielectric  & Plastic & Diffuse  \\ % \hline
        \vspace{-5pt} \\
        \rotatebox{90}{\parbox{\imghe}{\centering RGB Image}} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/gt_conductor_symmetrical_garden_4k_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/gt_dielectric_symmetrical_garden_4k_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/gt_plastic_symmetrical_garden_4k_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/gt_diffuse_symmetrical_garden_4k_10.png} \\
        % PGSR_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_roughplastic_10.png
        \rotatebox{90}{\parbox{\imghe}{\centering PGSR}} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/PGSR_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_conductor_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/PGSR_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_dielectric_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/PGSR_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_plastic_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/PGSR_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_diffuse_10.png} \\

        \rotatebox{90}{\parbox{\imghe}{\centering NeRO}} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/NeRO_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_conductor_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/NeRO_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_dielectric_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/NeRO_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_plastic_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/NeRO_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_diffuse_10.png} \\
        
        \rotatebox{90}{\parbox{\imghe}{\centering 2DGS}} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/2dgs_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_conductor_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/2dgs_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_dielectric_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/2dgs_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_plastic_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/2dgs_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_diffuse_10.png} \\
        
        \rotatebox{90}{\parbox{\imghe}{\centering Instant-NeuS}} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/instant-nsr-pl-wmask_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_conductor_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/instant-nsr-pl-wmask_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_dielectric_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/instant-nsr-pl-wmask_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_plastic_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/instant-nsr-pl-wmask_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_diffuse_10.png} \\
        
        \rotatebox{90}{\parbox{\imghe}{\centering NeuS2}} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/neus2_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_conductor_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/neus2_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_dielectric_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/neus2_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_plastic_10.png} &
        \includegraphics[width=.24\textwidth]{img/ablation_neus_2/neus2_5c230ea126b943b8bc1da3f5865d5cd2_symmetrical_garden_4k_diffuse_10.png} \\
        
    \end{tabular}
    \caption{\label{fig:neus_appendix-ablation} \textbf{Additional qualitative 3D reconstruction results on the ablation dataset.}}
    \end{minipage}
\end{figure*}

==> fig/reconstruction_2.tex <==
\begin{figure*}[htb]
    % \setlength{\belowcaptionskip}{-10pt}
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{cccc}
        Image & GT shape  & PGSR &  NeRO  \\
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_df894b66e2e54b558a43497becb94ff0-conductor.png} & % name should be 2d_gt_XXXX.png
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_df894b66e2e54b558a43497becb94ff0_11.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/PGSR_df894b66e2e54b558a43497becb94ff0_11.png}&
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/NeRO_df894b66e2e54b558a43497becb94ff0_11.png} \\
        
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_a2210a0ba6834141af3bf83ee1e03f07-dielectric.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/gt_a2210a0ba6834141af3bf83ee1e03f07_3.png} &
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/PGSR_a2210a0ba6834141af3bf83ee1e03f07_3.png}&
        \includegraphics[width=.24\textwidth]{img/vis-neus-c/NeRO_a2210a0ba6834141af3bf83ee1e03f07_3.png}\\

    \end{tabular}
    \caption{\label{fig:neus} \textbf{Qualitative 3D reconstruction results.} Top row: Input images; Second row: Ground truth; Third row: PGSR\cite{Chen24}; Bottom row: NeRO\cite{Liu23b}.}
\end{figure*}


==> fig/shape-ablation.tex <==
\newcommand{\imghei}{.135\textwidth}
\begin{figure*}[htb]
    \setlength{\belowcaptionskip}{-.5cm}
    \centering
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{2pt}
    \begin{minipage}{\textwidth}
    \begin{tabular}{cccccc}
        & Vase & Snail  & Boat & Motor Bike & Statue \\ % \hline
        \vspace{-5pt} \\
        \rotatebox{90}{\parbox{\imghei}{\centering RGB Image}} &
        \includegraphics[width=.18\textwidth]{img/ablation-preview/b14a251fe8ad4a10bbc75f7dd3f6cebb/gt_conductor_leadenhall_market_4k_12.png} &
        \includegraphics[width=.18\textwidth]{img/ablation-preview/fc4f34dae22c4dae95c19b1654c3cb7e/leadenhall_market_4k-conductor.png} &
        \includegraphics[width=.18\textwidth]{img/ablation-preview/01098ad7973647a9b558f41d2ebc5193/leadenhall_market_4k-conductor.png} &
        \includegraphics[width=.18\textwidth]{img/ablation-preview/df894b66e2e54b558a43497becb94ff0/leadenhall_market_4k-conductor.png} &
        \includegraphics[width=.18\textwidth]{img/ablation-preview/5c230ea126b943b8bc1da3f5865d5cd2/leadenhall_market_4k-conductor.png} \\
        
        \rotatebox{90}{\parbox{\imghei}{\centering Shape}} &
        \includegraphics[width=.18\textwidth]{img/shape-ablation/gt_b14a251fe8ad4a10bbc75f7dd3f6cebb_12.png} &
        \includegraphics[width=.18\textwidth]{img/shape-ablation/gt_fc4f34dae22c4dae95c19b1654c3cb7e_31.png} &
        \includegraphics[width=.18\textwidth]{img/shape-ablation/gt_01098ad7973647a9b558f41d2ebc5193_0.png} &
        \includegraphics[width=.18\textwidth]{img/shape-ablation/gt_df894b66e2e54b558a43497becb94ff0_1.png} &
        \includegraphics[width=.18\textwidth]{img/shape-ablation/gt_5c230ea126b943b8bc1da3f5865d5cd2_10.png} \\

    \end{tabular}
    \caption{\label{fig:shape_appendix} \textbf{Selection of objects in the ablation dataset.}}
    \end{minipage}
\end{figure*}

==> table/ablation/lighting.tex <==
\begin{table}[htb]  
\centering  
\scriptsize  
\caption{\label{tab:ablation_light}\textbf{Ablation of Lighting Condition.}}  
\setlength{\tabcolsep}{20pt}  
\begin{tabular}{p{1.2cm}|c|ccc}  
\toprule  
\multirow{2}{*}{Metric} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{\textbf{Lighting Type}} \\  
                       &                         & street night & market hall & garden \\  
\midrule


\multirow{5}{*}{\parbox{1.2cm}{\centering Chamfer Distance$\downarrow$}}
                        & 2DGS~\cite{Huang24}             & \num{1.4259}                          & \num{1.3740}                         & \num{1.3371} \\
                        & Instant-NeuS~\cite{Guo22}              & \cellcolor{top3}\num{1.03488}          & \num{1.099435}                         & \num{1.106376}\\
                        & NeuS2~\cite{Wang23a}                     & \cellcolor{top2}\num{0.9680}          & \cellcolor{top3}\num{1.0118}         & \cellcolor{top3}\num{1.0299}\\
                        & PGSR~\cite{Chen24}                      & \cellcolor{top1}\num{0.8455}          & \cellcolor{top1}\num{0.9160}         & \cellcolor{top1}\num{0.8487}\\
                        & NeRO$\star$~\cite{Liu23b}                      & \num{1.0614}                          & \cellcolor{top2}\num{0.9669}         & \cellcolor{top2}\num{1.0003}\\
                        % & NeRRF$\star$ & 0.9062            & 0.9020            & 0.8916 \\
\midrule  
\multirow{7}{*}{\parbox{1.2cm}{\centering PSNR$\uparrow$}}         
                       & Gaussian Splatting~\cite{Kerbl23}          & \num{29.353405}        & \num{29.170987}           & \num{29.077644} \\
                       & InstantNGP~\cite{Muller22}  & \cellcolor{top2}\num{29.810709} & \num{28.92153} & \cellcolor{top3}\num{29.598134} \\
                       & 2DGS~\cite{Huang24}                    & \num{29.465541}        &    \num{28.803827}         &    \num{28.718458} \\
                       & PGSR~\cite{Chen24}                    & \cellcolor{top1}\num{29.841052}            &\cellcolor{top2}\num{29.491238}             &\cellcolor{top2}\num{29.660042}\\
                       & GES~\cite{Hamdi24}                     & \num{29.460795} & \cellcolor{top3}\num{29.292089} & \num{29.186757} \\
                       & GSDR$\star$~\cite{Ye24}        & \cellcolor{top3}\num{29.751078}        &    \cellcolor{top1}\num{29.749379}         &    \cellcolor{top1}\num{30.460075} \\  
                       & GaussianShader$\star$~\cite{Jiang23} & \num{21.306568} & \num{21.947638} & \num{22.570275} \\
                       
\bottomrule
\end{tabular}
\end{table}

==> table/ablation/lighting_nerf.tex <==
\begin{table}[htb]  
\centering  
\footnotesize  
\caption{\label{tab:ab_light_nerf}\textbf{Ablation of Lighting: Comparison of SOTA Novel View Synthesis Methods.(PSNR)}}  
\setlength{\tabcolsep}{9pt}  
\begin{tabular}{c|ccc}  
\toprule  
\multirow{2}{*}{Method} & \multicolumn{3}{c}{\textbf{Lighting Type}} \\  
                        &  Street Night & Market Hall & Garden \\  
\midrule      
Gaussian Splatting          & \num{29.353405}        & \num{29.170987}           & \num{29.077644} \\
InstantNGP  & \cellcolor{top2}\num{29.810709} & \num{28.92153} & \cellcolor{top3}\num{29.598134} \\
2DGS                    & \num{29.465541}        &    \num{28.803827}         &    \num{28.718458} \\
GSDR~\cite{Ye24}        & \cellcolor{top3}\num{29.751078}        &    \cellcolor{top1}\num{29.749379}         &    \cellcolor{top1}\num{30.460075} \\  
GaussianShader & \num{21.292661} & \num{21.632296} & \num{22.533689} \\
PGSR                    & \cellcolor{top1}\num{29.841052}            &\cellcolor{top2}\num{29.491238}             &\cellcolor{top2}\num{29.660042}\\
GES                     & \num{29.418592} & \cellcolor{top3}\num{29.338640} & \num{29.163877} \\

\bottomrule  
\end{tabular}  
\end{table}


\begin{comment}
\begin{table*}[htb]  
\centering  
\footnotesize  
\caption{\label{tab:ab_light_nerf}\textbf{Ablation of Lighting: Comparison of SOTA Novel View Synthesis Methods.}}  
\setlength{\tabcolsep}{3pt}  
\begin{tabular}{c|c|ccc}  
\toprule  
\multirow{2}{*}{Metric} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{\textbf{Lighting Type}} \\  
                       &                         & street night & market hall & garden \\  
\midrule  
\multirow{2}{*}{PSNR$\uparrow$}        
                       & Gaussian Splatting          & \num{29.353405}        & \num{29.170987}           & \num{29.077644} \\
                       & InstantNGP  & \cellcolor{top2}\num{29.810709} & \num{28.92153} & \cellcolor{top3}\num{29.598134} \\
                       & 2DGS                    & \num{29.465541}        &    \num{28.803827}         &    \num{28.718458} \\
                       & GSDR~\cite{Ye24}        & \cellcolor{top3}\num{29.751078}        &    \cellcolor{top1}\num{29.749379}         &    \cellcolor{top1}\num{30.460075} \\  
                       & GaussianShader & \num{21.292661} & \num{21.632296} & \num{22.533689} \\
                       & PGSR                    & \cellcolor{top1}\num{29.841052}            &\cellcolor{top2}\num{29.491238}             &\cellcolor{top2}\num{29.660042}\\
                       & GES                     & \num{29.418592} & \cellcolor{top3}\num{29.338640} & \num{29.163877} \\
\midrule  
\multirow{2}{*}{SSIM$\uparrow$}        
                       & Gaussian Splatting          & \num{0.928556}         & \num{0.921995}            & \num{0.924404} \\
                       & InstantNGP  & \cellcolor{top3}\num{0.936667} & \num{0.926708} & \cellcolor{top3}\num{0.935646} \\
                       & 2DGS                    & \num{0.913261}        &     \num{0.895961}         &     \num{0.897869} \\
                       & GSDR                    & \cellcolor{top2}\num{0.946881}       &      \cellcolor{top2}\num{0.938348}          &     \cellcolor{top2}\num{0.944310} \\  
                       & GaussianShader & \num{0.894371} & \num{0.880551} & \num{0.895449} \\
                       & PGSR                    &\cellcolor{top1}\num{0.950011}            & \cellcolor{top1}\num{0.938923}              &\cellcolor{top1}\num{0.946201}\\
                       & GES                     & \num{0.931426} & \cellcolor{top3}\num{0.927501} & \num{0.928382} \\
\midrule  
\multirow{2}{*}{LPIPS$\downarrow$}     
                       & Gaussian Splatting          & \num{0.073420}          & \num{0.073679}            & \num{0.072303} \\
                       & InstantNGP  & \num{0.093044} & \num{0.100124} & \num{0.093898} \\
                       & 2DGS                    & \cellcolor{top2}\num{0.071511}        &     \num{0.076641}          &    \num{0.075242} \\
                       & GSDR                    & \cellcolor{top3}\num{0.072700}         &    \cellcolor{top3}\num{0.073483}           &   \cellcolor{top2}\num{0.070095} \\  
                       & GaussianShader & \num{0.154443} & \num{0.155293} & \num{0.150949} \\
                       & PGSR                    & \cellcolor{top1}\num{0.067757}             & \cellcolor{top1}\num{0.071440}             & \cellcolor{top1}\num{0.066178} \\
                       & GES                     & \num{0.073852} & \cellcolor{top2}\num{0.073021} & \cellcolor{top3}\num{0.071910} \\
\bottomrule  
\end{tabular}  
\end{table*}
\end{comment}

==> table/ablation/lighting_neus.tex <==
\begin{table}[ht]
\centering
\footnotesize
\caption{\label{tab:ab_light_neus}\textbf{Ablation of Lighting: Comparison of SOTA 3D Reconstruction Methods.} We report the Chamfer distance $\times 10^{-2}$.}
\setlength{\tabcolsep}{12pt}
\begin{tabular}{c|cccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c}{\textbf{Lighting Type}} \\
                          &  Street Night & Market Hall & Garden  \\
\midrule

2DGS~\cite{Huang24}       & \num{1.4259}                          & \num{1.3740}                         & \num{1.3371} \\
NeRO                      & \num{1.0805}                          & \cellcolor{top2}\num{0.9669}         & \cellcolor{top2}\num{1.0003}\\
Instant-NeuS              & \cellcolor{top3}\num{1.0350}          & \num{1.1204}                         & \num{1.1248}\\
NeuS2                     & \cellcolor{top2}\num{0.9680}          & \cellcolor{top3}\num{1.0118}         & \cellcolor{top3}\num{1.0299}\\
PGSR                      & \cellcolor{top1}\num{0.8455}          & \cellcolor{top1}\num{0.9160}         & \cellcolor{top1}\num{0.8487}\\
\bottomrule
\end{tabular}
\end{table}


\begin{comment}
\begin{table*}[ht]
\centering
% \scriptsize
\caption{\label{tab:ab_light_neus}\textbf{Comparison of SOTA 3D Reconstruction Methods.} We report the Chamfer distance $\times 10^{-2}$.}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{c|cccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c}{\textbf{Material Type}} \\
                          &  street night & market hall & garden  \\
\midrule

2DGS~\cite{Huang24}       & \num{1.425899}                          & \num{1.373982}                         & \num{1.337124} \\
NeRO                      & \num{1.080533}                          & \cellcolor{top2}\num{0.966852}         & \cellcolor{top2}\num{1.000311}\\
Instant-NeuS              & \cellcolor{top3}\num{1.034969}          & \num{1.120432}                         & \num{1.124752}\\
NeuS2                     & \cellcolor{top2}\num{0.968046}          & \cellcolor{top3}\num{1.011797}         & \cellcolor{top3}\num{1.029901}\\
PGSR                      & \cellcolor{top1}\num{0.845462}          & \cellcolor{top1}\num{0.916003}         & \cellcolor{top1}\num{0.84872}\\
\bottomrule
\end{tabular}
\end{table*}
\end{comment}

==> table/ablation/material_nerf.tex <==
\begin{table*}[htb]  
\centering  
\footnotesize  
\caption{\label{tab:ab_material_nerf}\textbf{Ablation of Material Type: Comparison of SOTA Novel View Synthesis Methods.(PSNR)}}  
\setlength{\tabcolsep}{5pt}  
\begin{tabular}{c|ccccccc}  
\toprule  
\multirow{2}{*}{Method} & \multicolumn{7}{c}{\textbf{Material Type}} \\  
                         & Conductor & Dielectric & Plastic & Rough Conductor & Rough Dielectric & Rough Plastic & Diffuse \\  
\midrule     
Gaussian Splatting      & \cellcolor{top2}\num{21.3856}    & \num{21.926318} & \cellcolor{top3}\num{34.161479}     & \num{28.112349}      & \num{28.425814}  & \num{35.124162}  & \cellcolor{top3}\num{35.269029} \\
Instant-NGP  & \num{21.038271} & \cellcolor{top2}\num{23.396643} & \num{34.104555} & \num{27.093283} & \cellcolor{top1}\num{30.985292} & \num{34.714689} & \num{34.771471}\\
2DGS                    & \num{19.926959}  &  \num{20.41677} &  \cellcolor{top1}\num{35.595247}    &  \num{24.851087}     &  \num{28.475166}  &  \cellcolor{top1}\num{36.523827}  & \cellcolor{top2}\num{37.182538}\\
GSDR~\cite{Ye24}        & \num{21.278171}  & \cellcolor{top3}\num{22.729077} & \cellcolor{top2}\num{34.956552}     & \cellcolor{top3}\num{28.135336}      & \cellcolor{top3}\num{29.295549}  &  \cellcolor{top2}\num{36.148513}  & \cellcolor{top1}\num{37.36471} \\ 
GaussianShader          & \num{18.054116} & \num{20.543025} & \num{23.675352} & \num{20.443618} & \num{23.240777} & \num{23.212869} & \num{23.916294} \\
PGSR                    & \cellcolor{top3}\num{21.286408}  & \cellcolor{top1}\num{23.93008}  & \num{33.754025}     & \cellcolor{top1}\num{29.423777}      & \cellcolor{top2}\num{30.400894}  & \num{34.397354}  & \num{34.456235} \\
GES                     & \cellcolor{top1}\num{21.476255} & \num{22.163985} & \num{34.069823} & \cellcolor{top2}\num{28.478768} & \num{28.636069} & \cellcolor{top3}\num{35.157679} & \num{35.133738} \\
\bottomrule  
\end{tabular}  
\end{table*}

\begin{comment}

% Here is the full table, will be moved to the supplementary.

\begin{table*}[htb]  
\centering  
\footnotesize  
\caption{\label{tab:ab_material_nerf}\textbf{Ablation of Material Type: Comparison of SOTA Novel View Synthesis Methods.}}  
\setlength{\tabcolsep}{3pt}  
\begin{tabular}{c|c|ccccccc}  
\toprule  
\multirow{2}{*}{Metric} & \multirow{2}{*}{Method} & \multicolumn{7}{c}{\textbf{Material Type}} \\  
                       &                         & Conductor & Dielectric & Plastic & Rough Conductor & Rough Dielectric & Rough Plastic & Diffuse \\  
\midrule  
\multirow{3}{*}{PSNR$\uparrow$}        
                       & Gaussian Splatting      & \cellcolor{top2}\num{21.3856}    & \num{21.926318} & \cellcolor{top3}\num{34.161479}     & \num{28.112349}      & \num{28.425814}  & \num{35.124162}  & \cellcolor{top3}\num{35.269029} \\
                       & Instant-NGP  & \num{21.038271} & \cellcolor{top2}\num{23.396643} & \num{34.104555} & \num{27.093283} & \cellcolor{top1}\num{30.985292} & \num{34.714689} & \num{34.771471}\\
                       & 2DGS                    & \num{19.926959}  &  \num{20.41677} &  \cellcolor{top1}\num{35.595247}    &  \num{24.851087}     &  \num{28.475166}  &  \cellcolor{top1}\num{36.523827}  & \cellcolor{top2}\num{37.182538}\\
                       & GSDR~\cite{Ye24}        & \num{21.278171}  & \cellcolor{top3}\num{22.729077} & \cellcolor{top2}\num{34.956552}     & \cellcolor{top3}\num{28.135336}      & \cellcolor{top3}\num{29.295549}  &  \cellcolor{top2}\num{36.148513}  & \cellcolor{top1}\num{37.36471} \\ 
                       & GaussianShader          & \num{18.054116} & \num{20.543025} & \num{23.675352} & \num{20.443618} & \num{23.240777} & \num{23.212869} & \num{23.916294} \\
                       & PGSR                    & \cellcolor{top3}\num{21.286408}  & \cellcolor{top1}\num{23.93008}  & \num{33.754025}     & \cellcolor{top1}\num{29.423777}      & \cellcolor{top2}\num{30.400894}  & \num{34.397354}  & \num{34.456235} \\
                       & GES                     & \cellcolor{top1}\num{21.476255} & \num{22.163985} & \num{34.069823} & \cellcolor{top2}\num{28.478768} & \num{28.636069} & \cellcolor{top3}\num{35.157679} & \num{35.133738} \\
\midrule  
\multirow{3}{*}{SSIM$\uparrow$}        
                       & Gaussian Splatting      & \num{0.827683}   & \num{0.827839}  & \num{0.975441}      & \num{0.937521}       & \num{0.940478}    & \num{0.98149}     & \num{0.984442} \\
                       & Instant-NGP  & \num{0.826894} & \cellcolor{top3}\num{0.852457} & \cellcolor{top3}\num{0.980267} & \num{0.936675} & \cellcolor{top3}\num{0.960709} & \cellcolor{top3}\num{0.985252} & \cellcolor{top3}\num{0.988796}\\
                       & 2DGS                    & \num{0.774781}   & \num{0.790641}  & \num{0.975009}      & \num{0.881812}       & \num{0.930911}    & \num{0.981532}    & \num{0.981862} \\
                       & GSDR                    & \cellcolor{top1}\num{0.85805}    & \cellcolor{top2}\num{0.857822}  & \cellcolor{top2}\num{0.983454}      & \cellcolor{top2}\num{0.9596}         & \cellcolor{top2}\num{0.963528}    & \cellcolor{top2}\num{0.98913}     & \cellcolor{top1}\num{0.990672} \\  
                       & GaussianShader          & \num{0.808936} & \num{0.829466} & \num{0.92876} & \num{0.886097} & \num{0.923826} & \num{0.927915} & \num{0.935767} \\
                       & PGSR                    & \cellcolor{top2}\num{0.845763}   & \cellcolor{top1}\num{0.868899}  & \cellcolor{top1}\num{0.984359}      & \cellcolor{top1}\num{0.966364}       & \cellcolor{top1}\num{0.970104}    & \cellcolor{top1}\num{0.989155}    & \cellcolor{top2}\num{0.990671} \\
                       & GES                     & \cellcolor{top3}\num{0.835068} & \num{0.835528} & \num{0.976466} & \cellcolor{top3}\num{0.943197} & \num{0.945466} & \num{0.982942} & \num{0.985012} \\                 
\midrule  
\multirow{3}{*}{LPIPS$\downarrow$}     
                       & Gaussian Splatting      & \cellcolor{top3}\num{0.13031}    & \num{0.134186}  & \cellcolor{top2}\num{0.042665}      & \num{0.069718}       & \num{0.079281}    & \cellcolor{top2}\num{0.029962}    & \cellcolor{top2}\num{0.025815} \\
                       & Instant-NGP  & \num{0.163106} & \num{0.146906} & \num{0.064511} & \num{0.108408} & \num{0.099000} & \num{0.052194} & \num{0.035697} \\
                       & 2DGS                    & \num{0.147963}   & \num{0.140433}  & \cellcolor{top1}\num{0.033903}      & \num{0.08712}        & \cellcolor{top2}\num{0.071023}    & \cellcolor{top1}\num{0.02193}     & \cellcolor{top1}\num{0.018879} \\
                       & GSDR                    & \cellcolor{top1}\num{0.124034}   & \cellcolor{top2}\num{0.131688}  & \cellcolor{top3}\num{0.043713}      & \cellcolor{top2}\num{0.066842}       & \num{0.080551}    & \cellcolor{top3}\num{0.03009}     & \num{0.027731} \\
                       & GaussianShader          & \num{0.17961} & \num{0.175211} & \num{0.139105} & \num{0.155863} & \num{0.149823} & \num{0.138612} & \num{0.134106} \\
                       & PGSR                    & \cellcolor{top2}\num{0.129042}   & \cellcolor{top1}\num{0.115571}  & \num{0.044028}      & \cellcolor{top1}\num{0.061464}       & \cellcolor{top1}\num{0.069256}    & \num{0.032122}    & \num{0.027726} \\
                       & GES                     & \num{0.13102} & \cellcolor{top3}\num{0.134102} & \num{0.044125} & \cellcolor{top3}\num{0.067131} & \cellcolor{top3}\num{0.076073} & \num{0.030747} & \cellcolor{top3}\num{0.02707} \\
\bottomrule  
\end{tabular}  
\end{table*}
\end{comment}



==> table/ablation/material_neus.tex <==
\begin{table*}[ht]
\centering
\footnotesize  
\caption{\label{tab:ab_material_neus}\textbf{Ablation of Material Type: Comparison of SOTA 3D Reconstruction Methods.} We report the Chamfer distance $\times 10^{-2}$.}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{c|cccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{7}{c}{\textbf{Material Type}} \\
                          & Conductor  & Dielectric & Plastic  & Rough Conductor & Rough Dielectric    & Rough Plastic & Diffuse\\
\midrule

2DGS~\cite{Huang24}       & \num{2.0784}                 & \num{1.8583}                 & \cellcolor{top3}\num{0.6116}     & \num{1.7614}                    & \num{1.6913}                        & \cellcolor{top3}\num{0.5903}    & \cellcolor{top3}\num{0.5565} \\
NeRO                      & \cellcolor{top1}\num{0.7802} & \num{1.9700}                 & \cellcolor{top2}\num{0.5523}     & \cellcolor{top1}\num{0.7483}    & \num{1.5726}                        & \cellcolor{top2}\num{0.5514}    & \cellcolor{top1}\num{0.4710} \\
Instant-NeuS              & \num{1.5373}                 & \cellcolor{top3}\num{1.3668} & \num{0.6184}                     & \num{1.4574}                    & \cellcolor{top3}\num{1.3164}        & \num{0.6033}                    & \num{0.5749} \\
NeuS2                     & \cellcolor{top3}\num{1.4161} & \cellcolor{top2}\num{1.1342} & \num{0.6483}                     & \cellcolor{top3}\num{1.2518}    & \cellcolor{top2}\num{1.0931}        & \num{0.6322}                    & \num{0.6256} \\
PGSR                      & \cellcolor{top2}\num{1.3137} & \cellcolor{top1}\num{0.9845} & \cellcolor{top1}\num{0.5063}     & \cellcolor{top2}\num{1.0403}    & \cellcolor{top1}\num{0.9267}        & \cellcolor{top1}\num{0.4807}    & \cellcolor{top2}\num{0.4814} \\

\bottomrule
\end{tabular}
\end{table*}


\begin{comment}
\begin{table*}[ht]
\centering
% \scriptsize
\caption{\label{tab:ab_material_neus}\textbf{Comparison of SOTA 3D Reconstruction Methods.} We report the Chamfer distance $\times 10^{-2}$.}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{c|cccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{7}{c}{\textbf{Material Type}} \\
                          & Conductor  & Dielectric & Plastic  & Rough Conductor & Rough Dielectric    & Rough Plastic & Diffuse\\
\midrule

2DGS~\cite{Huang24}       &\num{2.078354}   &\num{1.858319}  &\num{0.611589}       &\num{1.761405}        & \num{1.69133}   &  \num{0.590311}  & \num{0.556489} \\
NeRO                      & \num{0.780223}   &\num{1.970044}  &\num{0.552273}        &\num{0.74827}       & \num{1.572633}    & \num{0.551398} & \num{0.470993} \\
Instant-NeuS              & \num{1.537295}  & \num{1.366834}  &\num{0.618362}       &\num{1.457431}      &  \num{1.316434}    & \num{0.603257} & \num{0.574948} \\
NeuS2                     &\num{1.416088}   & \num{1.134237}  &\num{0.648267}       &\num{1.251756}       & \num{1.093085}   &  \num{0.632198} & \num{0.625555} \\
PGSR                      & \num{1.313654}   & \num{0.98453}  &\num{0.506311}       &\num{1.040275}        &\num{0.926706}    & \num{0.480733}  &\num{0.481442} \\

\bottomrule
\end{tabular}
\end{table*}
\end{comment}



==> table/ablation/shape_nerf.tex <==
\begin{table}[htb]  
\centering  
\footnotesize  
\caption{\label{tab:ab_shape_nerf}\textbf{Ablation of Geometry Shape: Comparison of SOTA Novel View Synthesis Methods.(PSNR)}}  
\setlength{\tabcolsep}{3pt}  
\begin{tabular}{c|ccccc}  
\toprule  
\multirow{2}{*}{Method} & \multicolumn{5}{c}{\textbf{Object Name}} \\  
                        & Vase  & Snail & Boat  & Motor Bike & Statue  \\  
\midrule  
Gaussian Splatting          & \num{28.855678}  & \num{29.161615} & \num{29.409573}  & \cellcolor{top3}\num{28.781895}  & \num{29.794633} \\
Instant-NGP  & \cellcolor{top1}\num{29.962749}  & \cellcolor{top3}\num{30.145689}  & \num{28.940783}  & \num{28.38213}  & \num{29.785938} \\
2DGS                    & \num{24.921071} & \cellcolor{top1}\num{30.796852}  & \cellcolor{top2}\num{30.436085} & \num{28.564278} & \cellcolor{top3}\num{30.261425} \\
GSDR~\cite{Ye24}        & \num{28.795018} & \num{29.994795}  & \cellcolor{top1}\num{30.693927} & \cellcolor{top1}\num{29.373514} & \cellcolor{top1}\num{31.076965} \\  
GaussianShader & \num{22.473356} & \num{21.208088} & \num{22.683831} & \num{20.344479} & \num{22.62829} \\
PGSR                    & \cellcolor{top2}\num{29.244217} & \cellcolor{top2}\num{30.232075} & \num{29.131888} & \cellcolor{top2}\num{29.223300} & \cellcolor{top2}\num{30.489071} \\
GES & \cellcolor{top3}\num{29.047588} & \num{29.289801} & \cellcolor{top3}\num{29.624691} & \num{28.70121} & \num{30.121383} \\

\bottomrule  
\end{tabular}  
\end{table}



\begin{comment}

\begin{table*}[htb]  
\centering  
\footnotesize  
\caption{\label{tab:ab_shape_nerf}\textbf{Ablation of Geometry Shape: Comparison of SOTA Novel View Synthesis Methods.}}  
\setlength{\tabcolsep}{3pt}  
\begin{tabular}{c|c|ccccc}  
\toprule  
\multirow{2}{*}{Metric} & \multirow{2}{*}{Method} & \multicolumn{5}{c}{\textbf{Object Name}} \\  
                       &                         & vase & snail & Boat & Bike & Statue  \\  
\midrule  
% 'b14a251fe8ad4a10bbc75f7dd3f6cebb': "vase",
% 'fc4f34dae22c4dae95c19b1654c3cb7e': "snail",
% '01098ad7973647a9b558f41d2ebc5193': "Boat",
% 'df894b66e2e54b558a43497becb94ff0': "Bike",
% '5c230ea126b943b8bc1da3f5865d5cd2': "Statue",
\multirow{3}{*}{PSNR$\uparrow$}  
                       & Gaussian Splatting          & \num{28.855678}  & \num{29.161615} & \num{29.409573}  & \cellcolor{top3}\num{28.781895}  & \num{29.794633} \\
                       & Instant-NGP  & \cellcolor{top1}\num{29.962749}  & \cellcolor{top3}\num{30.145689}  & \num{28.940783}  & \num{28.38213}  & \num{29.785938} \\
                       & 2DGS                    & \num{24.921071} & \cellcolor{top1}\num{30.796852}  & \cellcolor{top2}\num{30.436085} & \num{28.564278} & \cellcolor{top3}\num{30.261425} \\
                       & GSDR~\cite{Ye24}        & \num{28.795018} & \num{29.994795}  & \cellcolor{top1}\num{30.693927} & \cellcolor{top1}\num{29.373514} & \cellcolor{top1}\num{31.076965} \\  
                       & GaussianShader & \num{22.473356} & \num{21.208088} & \num{22.683831} & \num{20.344479} & \num{22.62829} \\
                       & PGSR                    & \cellcolor{top2}\num{29.244217} & \cellcolor{top2}\num{30.232075} & \num{29.131888} & \cellcolor{top2}\num{29.223300} & \cellcolor{top2}\num{30.489071} \\
                       & GES & \cellcolor{top3}\num{29.047588} & \num{29.289801} & \cellcolor{top3}\num{29.624691} & \num{28.70121} & \num{30.121383} \\
\midrule  
\multirow{3}{*}{SSIM$\uparrow$}        
                       & Gaussian Splatting          & \num{0.924165}   & \num{0.910944} & \num{0.945255}   & \num{0.915406}   & \num{0.929154} \\
                       & Instant-NGP  & \cellcolor{top3}\num{0.936083}  & \cellcolor{top3}\num{0.927871}  & \cellcolor{top2}\num{0.950387} & \num{0.917707} & \num{0.932986} \\
                       & 2DGS                    & \num{0.869839}  & \num{0.910252} & \num{0.932386}  & \num{0.890244}  & \num{0.909098}  \\
                       & GSDR                    & \cellcolor{top1}\num{0.942138}  & \cellcolor{top2}\num{0.936362} & \cellcolor{top1}\num{0.96244}   & \cellcolor{top2}\num{0.932939}  & \cellcolor{top2}\num{0.942019}  \\ 
                       & GaussianShader  & \num{0.904208} & \num{0.897032} & \num{0.916698} & \num{0.860365} & \num{0.879074} \\
                       & PGSR                    & \cellcolor{top2}\num{0.936534}  & \cellcolor{top1}\num{0.959603}  & \num{0.94325} & \cellcolor{top1}\num{0.937554}  & \cellcolor{top1}\num{0.948284}  \\
                       & GES & \num{0.929576} & \num{0.916403} & \cellcolor{top3}\num{0.949242} & \cellcolor{top3}\num{0.918101} & \cellcolor{top3}\num{0.933695} \\
\midrule  
\multirow{3}{*}{LPIPS$\downarrow$}     
                       & Gaussian Splatting          & \cellcolor{top2}\num{0.083097}   & \num{0.088063} & \num{0.056139}   & \cellcolor{top3}\num{0.071905}   & \cellcolor{top3}\num{0.066466}  \\
                       & Instant-NGP  & \num{0.11438}  & \num{0.110278}  & \num{0.07256}  & \num{0.09933}  & \num{0.081896} \\
                       & 2DGS                    & \num{0.104201}  & \cellcolor{top1}\num{0.075824} & \cellcolor{top2}\num{0.054059}  & \num{0.074663}  & \cellcolor{top2}\num{0.063575}  \\
                       & GSDR                    & \cellcolor{top3}\num{0.083178}  & \cellcolor{top3}\num{0.086016} & \cellcolor{top1}\num{0.052013}  & \cellcolor{top2}\num{0.071135}  & \num{0.068121}  \\ 
                       & GaussianShader & \num{0.150213} & \num{0.170665} & \num{0.119214} & \num{0.178593} & \num{0.147673} \\
                       & PGSR                    & \num{0.084794}  & \cellcolor{top2}\num{0.077382} & \cellcolor{top3}\num{0.054694}  & \cellcolor{top1}\num{0.064427}  & \cellcolor{top1}\num{0.060995}  \\
                       & GES & \cellcolor{top1}\num{0.081418} & \num{0.086394} & \cellcolor{top3}\num{0.054738} & \num{0.072587} & \num{0.067563} \\                 
\bottomrule  
\end{tabular}  
\end{table*}
\end{comment}

==> table/ablation/shape_neus.tex <==
\begin{table}[ht]
\centering
\footnotesize  
\caption{\label{tab:ab_shape_neus}\textbf{Ablation of Geometry Shape: Comparison of SOTA 3D Reconstruction Methods.} We report the Chamfer distance $\times 10^{-2}$.}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{c|cccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c}{\textbf{Object Name}} \\
                          & Vase  & Snail & Boat  & Motor Bike & Statue  \\
\midrule        
% 'b14a251fe8ad4a10bbc75f7dd3f6cebb': "vase",
% 'fc4f34dae22c4dae95c19b1654c3cb7e': "snail",
% '01098ad7973647a9b558f41d2ebc5193': "Boat",
% 'df894b66e2e54b558a43497becb94ff0': "Bike",
% '5c230ea126b943b8bc1da3f5865d5cd2': "Statue",
2DGS~\cite{Huang24}       & \num{1.8806}                  & \num{2.1451} & \cellcolor{top1}\num{0.7352}   & \num{1.0741}                   & \num{1.0600}                  \\
NeRO                      & \cellcolor{top1}\num{1.2317}  & \cellcolor{top3}\num{1.1328} & \num{1.1276}                   & \num{1.0740}                   & \cellcolor{top2}\num{0.5159}  \\
Instant-NeuS              & \cellcolor{top2}\num{1.2361}  & \num{1.4497} & \cellcolor{top3}\num{1.0065}   & \cellcolor{top3}\num{0.9656}   & \num{0.8034}                  \\
NeuS2                     & \num{1.3190}                  & \cellcolor{top1}\num{1.0958} & \num{1.0867}                   & \cellcolor{top2}\num{0.9655}   & \cellcolor{top3}\num{0.5492}  \\
PGSR                     & \cellcolor{top3}\num{1.2407}  & \cellcolor{top2}\num{1.1155}  & \cellcolor{top2}\num{0.8168}   & \cellcolor{top1}\num{0.8779}   & \cellcolor{top1}\num{0.2995}  \\
        
\bottomrule
\end{tabular}
\end{table}

\begin{comment}
\begin{table*}[ht]
\centering
% \scriptsize
\caption{\label{tab:ab_shape_neus}\textbf{Comparison of SOTA 3D Reconstruction Methods.} We report the Chamfer distance $\times 10^{-2}$.}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{c|cccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c}{\textbf{Material Type}} \\
                          & obj 1  & obj 2 & obj 3  & obj 4 & obj 5  \\
\midrule
% obj in order: 5c230ea126b943b8bc1da3f5865d5cd2 01098ad7973647a9b558f41d2ebc5193 b14a251fe8ad4a10bbc75f7dd3f6cebb df894b66e2e54b558a43497becb94ff0 fc4f34dae22c4dae95c19b1654c3cb7e
2DGS~\cite{Huang24}       & \num{1.059998}  & \num{0.735239}   &\num{1.880625}           & \num{1.074069}     &\num{2.145078} \\
NeRO                      & \num{0.515949}  & \num{1.127561}   &   \num{1.231679}     &    \num{1.073996}   &      \num{1.132798} \\
Instant-NeuS              & \num{0.8034}    & \num{1.006455}   &   \num{1.236101}   &   \num{0.965645}     &     \num{1.449687} \\
NeuS2                     & \num{0.549228}  & \num{1.08673}    &    \num{1.319017}   &    \num{0.965472}   &     \num{1.095794} \\
PGSR                      & \num{0.299478}  & \num{0.816793}     &   \num{1.240678}   &   \num{0.877898}    &     \num{1.115462} \\

\bottomrule
\end{tabular}
\end{table*}
\end{comment}



    
        

==> table/dataset.tex <==
% foucus on the dataset with only images

% synthetic and real, real only few objecy

% realistic rendering , physic based rendering,

% material, categories

% data source

% 




\begin{table}[h]
\centering

\caption{Comparison with Existing Object-centric Inverse Rendering Datasets.
*Objaverse consists of both synthetic objects and real scans. 
%
}
%
\scriptsize
\begin{tabular}{lccccccccc}
\toprule
Dataset & \# Scenes & \# Objects & Real & Scene Type & Multi-view & Shape  & Relit Image  & Lighting & Material type \\
% list out all the datasets in the NeRF area.
\midrule
MIT Intrinsics      & 1     & 20     & \yes    & \studio         &\yes  & \no  & \no  & \no  & - \\
DTU-MVS             & 1     & 80     & \yes    & \studio         &\yes  & \yes & \no  & \no  & - \\
Objaverse           & 818K  & 818K   & (\yes)* & \studio         &\yes  & \yes & \no  & \no  & -\\
DiLiGenT-MV         & 1     & 5      & \yes    & \studio         &\yes  & \yes & \yes & \yes & - \\
ReNe                & 1     & 20     & \yes    & \studio         &\yes  & \no  & \yes & \yes & - \\
OpenIllumination    & 155   & 64     & \yes    & \studio         &\yes  & \no  & \yes & \yes & -\\
Lombardi            & 5     & 6      & \yes    & \wild           &\no   & \yes & \yes & \yes & - \\
NeRD Real           & 4     & 4      & \yes    & \wild           &\yes  & \no  & \yes & \no  & - \\
NeROIC              & 10    & 3      & \yes    & \wild           &\yes  & \no  & \yes & \no  & - \\
Oxholm              & 3     & 4      & \yes    & \wild           &\yes  & \yes & \yes & \yes & -\\
Stanford-ORB        & 7     & 14     & \yes    & \wild           &\yes  & \yes & \yes & \yes & - \\
NeRO-Dataset        & -     & -      & -       & -               & -    & -    & -    & -    & - \\
LLFF                & -     & -      & -       & -               & -    & -    & -    & -    & - \\
% NeRF original paper datset
Synthetic 360       & -     & -      & -       & -               & -    & -    & -    & -    & - \\
BlendedMVS          & -     & -      & -       & -               & -    & -    & -    & -    & - \\
\midrule
ShapeNet-Intrinsics & 98    & 31K    & \no     & \synthetic      &\yes  & \yes & \yes & \yes & - \\
NeRD Synthetic      & 30    & 3      & \no     & \synthetic      &\yes  & \yes & \yes & \yes & - \\
ABO                 & 40K   & 8K     & \no     & \synthetic      &\yes  & \yes & \yes & \yes & -\\
Ours                & 700+  & 1001   & \no     & indoor\&outdoor &\yes  & \yes & -    & -    & - \\

\midrule
% Scene-level dataset(Just list them here)
% ScanNet           
% Tanks and Temples
% Matterport-3D
% Replica dataset
% KITTI
% Waymo Open Dataset
\bottomrule
\end{tabular}
\label{tab:datasets}
\end{table}

==> table/dataset_image.tex <==
\begin{table}[ht]
\centering

\caption{Comparison with Existing Object-centric MVS Datasets.
}

\footnotesize
\begin{tabular}{lcccccc}
\toprule
Dataset             & Scenes    & Objects   & Shape      & Capture           &  Material Types    & Material Source     \\
\midrule
OpenIllumination\cite{Liu24}    & 155       & 64        & \no        & camera                 &  mixed             &      real           \\
LLFF Real\cite{Mildenhall19}           & 24        & 24        &\no         & camera                &  mixed             &      real         \\ % scene level
NeRD Real\cite{Boss21}           & 4         & 4         & \no        & camera                 &  mixed             &      real           \\
% from Ref-NeRF
Ref-NeRF dataset\cite{Verbin22}    & 1         & 3         &\no         & camera                 &  mixed             &      real           \\
NeROIC\cite{Kuang22}              & 10        & 3         & \no        & camera                &  mixed             &      real           \\
ReNe\cite{Toschi23}                & 1         & 20        & \no        & camera                 &  mixed             &      real           \\
% ground-truth 3D models of the objects acquired using a laser light-stripe range ﬁnder and manually ﬁnished, 4 simple shapes
Oxholm-real\cite{Oxholm14}              & 3         & 4         & \yes       & camera                &  mixed             &      real           \\
% ground-truth point cloud of the object, acquired using depth sensor.
DTU-MVS\cite{Aanaes16}            & 1         & 80        & \yes       & camera                 &  mixed             &      real           \\
% this dataset contain 8 object, Ground-truth data was captured using an industrial laser scanner.
Tanks and Temples\cite{Knapitsch17}   & 14        & 14        & \yes       & camera                 &  mixed             &      real         \\ % scene level
% using SfM to get the 3D reconstuction result.
DiLiGenT-MV\cite{Li20b}         & 1         & 5         & \yes       & camera                 &  mixed             &      real           \\
Stanford-ORB\cite{Kuang23}        & 7         & 14        & \yes       & camera                 &  mixed             &      real           \\
OmniObject3D\cite{Wu23}        & 1         & 6k        & \yes       & camera                 &  mixed             &      real           \\
NeRO Glossy-Real\cite{Liu23b}    & 1         & 5         & \yes       & camera                &  mixed             &      real           \\

% NAVI: Category-Agnostic Image Collections with High-Quality 3D Shape and Pose Annotations
NAVI\cite{Jampani24}              & 35        & 36        & \yes       & camera                 &  mixed             &      real           \\
\midrule
% NeRF original paper datset
Diffuse Synthetic 360\cite{Mildenhall21}  & 1      & 4        &\no          & basic BRDF            &  Lambertian                 &  Human definition         \\
Realistic Synthetic 360\cite{Mildenhall21}       & 1         & 8        &\no        & basic BRDF        &  mixed            &  Human definition         \\
NeRD Synthetic\cite{Boss21}      & 30        & 3         & \no       & basic BRDF        &  mixed                 & Human definition           \\
% from Ref-NeRF
ShinyBlender\cite{Verbin22}        & 1         & 6         & \no       & basic BRDF                 &  reflective                 & Human definition         \\
ShapeNet-Intrinsics\cite{Shi17}    & 98        & 31K       & \yes       & basic BRDF                 &  reflective                 &  Human definition          \\
Oxholm-Synthetic\cite{Oxholm14}    & 5         & 10         & \yes       & basic BRDF                &  single(7)             &     Lab Measurements           \\
BlendedMVS\cite{Yao20}             & 113       & 113       & \yes       & basic BRDF                &  mixed             &    Human definition        \\
ABO\cite{Collins22}                 & 40k       & 8K        & \yes       & basic BRDF        &  mixed                 &  Human definition           \\
Objaverse\cite{Deitke23}           & 81      & 818K      & \yes       & basic BRDF                 &  mixed             &      Human definition           \\
NeRO Glossy-Blender\cite{Liu23b} & 1         & 8         & \yes       & basic BRDF                 & reflective                 &  Human definition         \\
Ours                & 734(HDR)      & 1001      & \yes       & taliored BxDFs    &  single(291)       & Lab Measurements    \\

\midrule

\bottomrule
\end{tabular}
\label{tab:datasets}
\end{table}
% Kuang23,Wu23,Liu23b,Jampani24
% Mildenhall21，Boss21，Verbin22

% Scene-level dataset(Just list them here)
% ScanNet           
% Tanks and Temples
% Matterport-3D
% Replica dataset
% KITTI
% Waymo Open Dataset

==> table/datasheet.tex <==
\begin{table*}[htb]
\centering
\small
\caption{\label{tab:datasheet}\textbf{Datasheet for OpenMaterial}}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l|p{10cm}}
\toprule
% \multicolumn{2}{c}{\textbf{Datasheet for OpenMaterial}} \\
Section & Details \\
\midrule
Motivation 
& 1. \textbf{For what purpose was the dataset created?} 
This dataset was created to facilitate quantitative evaluation of existing 3D reconstruction algorithms for objects with diverse and challenging materials. It will help to pave the way for the development of 3D reconstruction algorithm capable of handling complex material properties. \\
& 2. \textbf{What (other) tasks could the dataset be used for?}
Primarily designed for 3D reconstruction, this dataset has also demonstrated suitability for novel view synthesis. Furthermore, it may be applicable to object-level 6D pose estimation, as ground-truth camera poses are provided. \\
& 3. \textbf{Who created the dataset?} 
The dataset was collaboratively created by researchers from the Computer Vision Laboratory (CVLab) at École Polytechnique Fédérale de Lausanne (EPFL), Switzerland, and the Institute of Artificial Intelligence and Robotics (IAIR) Laboratory at Xi'an Jiaotong University, China.\\
% & 4. \textbf{Who funded the creation of the dataset?} 
% The creation of this dataset was funded by \ZD{[Funding Agency/Institution].}\\

\midrule
Composition 
& 1. \textbf{What do the instances that comprise the dataset represent (e.g., documents, photos, people, countries)?}
Each instance in the dataset represents a scene in the form of dense multi-view images. \\
& 2. \textbf{How many instances are there in total?}
The dataset comprises 1,001 distinct scenes. \\
& 3. \textbf{What data does each instance consist of?}
Each scene features a unique geometric shape, a randomly selected material type, and a randomly chosen lighting condition. Furthermore, each scene consists of 90 RGB images captured from specific viewpoints, accompanied by a relative camera pose, an object mask, a depth map, a material type, and shape annotations. \\
& 4. \textbf{Is there a label or target associated with each instance?}
Yes, each instance is labeled according to its [object]-[material]-[lighting condition] attributes. \\

\midrule
Collection Process 
&1. \textbf{How was the data collected?}
We utilized 3D shapes from the Objaverse dataset and High Dynamic Range Imaging (HDRI) environment maps from Polyhaven. Additionally, we incorporated laboratory-measured Index of Refraction (IOR) data from scientific papers within a physics-based rendering framework to create this comprehensive, realistic dataset featuring complex materials.\\

\midrule
Uses 
& 1. \textbf{For what tasks has the dataset been used?}
This dataset has been used for 3D reconstruction and novel view synthesis.\\
& 2. \textbf{Is there a repository that links to any or all papers or systems that use the dataset?}
Papers and projects using this dataset can be found at \href{https://christy61.github.io/openmaterial.github.io/}{OpenMaterial}.\\
\midrule
Distribution 
& 1. \textbf{How is the dataset distributed (e.g., tarball on website, API, GitHub)?}
The dataset is available for download at \href{https://christy61.github.io/openmaterial.github.io/}{OpenMaterial}.\\
& 2. \textbf{What license (if any) is the data distributed under?}
The dataset as a whole is licensed under the CC BY-NC 4.0 DEED. However, individual 3D object shapes within the dataset are subject to different licenses. For more details on each object's specific license, please refer to the Objaverse documentation.\\
\midrule
Maintenance 
& 1. \textbf{Who is supporting/hosting/maintaining the dataset?}
The dataset is maintained by the Computer Vision Laboratory (CVLab) at École Polytechnique Fédérale de Lausanne (EPFL). \\

& 2. \textbf{How can others report issues or contribute to the dataset?}
Issues can be reported and contributions can be made via the Hugging Face repository or by contacting us via email.\\

\bottomrule
\end{tabular}
\end{table*}



==> tex/6-checklist.tex <==
\section*{Checklist}
\begin{comment}
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\end{comment}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Please see~\cref{sec:limitations_and_conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{This project focuses building dataset for 3D reconstruction. We have not identified direct negative societal impacts stemming from this specific research.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{The experiments were conducted on the university cluster, utilizing around 40 NVIDIA V100 GPUs.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{\zd{The dataset as a whole is licensed under the CC BY-NC 4.0 DEED. However, individual 3D object shapes within the dataset are subject to different licenses. For more details on each object's specific license, please refer to Objaverse's documentation.}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{\zd{The dataset can be viewed and downloaded through the following link: \href{https://christy61.github.io/openmaterial.github.io/}{https://christy61.github.io/openmaterial.github.io/}.}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tex/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{comment}
    
%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%
\end{comment}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction clearly present the key contributions of the paper: (1) The introduction of OpenMaterial, a large-scale dataset for material-aware 3D reconstruction; (2) the use of physically-based simulation with measured IOR spectra; and (3) the benchmarking of 11 SOTA methods and ablation studies across material, shape, and lighting variations. These claims are directly supported by the methodology and results detailed in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discusses several limitations in Section~\ref{sec:limitations_and_conclusion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not include formal theoretical results or proofs. However, it does provide all necessary physical modeling assumptions and mathematical formulations (e.g., the use of BRDF models) to support the dataset generation and rendering process. These are clearly described and justified in the method section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper describes all necessary details to reproduce the main experiments, including dataset composition details, benchmark protocols, and implementation settings. Upon acceptance, we will release all associated data and code, including dataset generation scripts, benchmarking tools, and material IOR spectral data, to facilitate full reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide open access to the full dataset during the review process, including rendered images, geometry, camera poses, depth maps, and material annotations. The dataset is hosted on Huggingface and can be accessed via the following link: (\url{https://huggingface.co/datasets/EPFL-CVLab/OpenMaterial}). Upon acceptance, we will also release the associated codebase, including dataset generation scripts, benchmarking tools, and material IOR spectra, to ensure full reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides all necessary experimental details to understand and reproduce the results, including dataset composition, geometry, lighting and material variations, evaluation metrics, and benchmarked methods.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    % \item[] Justification: The paper focuses on benchmarking deterministic 3D reconstruction algorithms under controlled material, shape, and lighting conditions, where statistical variation is not the primary concern.
    \item[] Justification: The benchmark focuses on deterministic evaluation under controlled material, shape, and lighting conditions. While some algorithms may involve stochastic components (e.g., random initialization), the primary goal is to assess comparative performance under fixed settings. Therefore, statistical significance analysis (e.g., across multiple runs) is not the emphasis of this benchmark, though it could be a valuable direction for future work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our experiments focus on benchmarking existing 3D reconstruction methods. Since we use publicly available implementations, compute requirements can be referred to in the original papers.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The dataset focuses on geometric object reconstruction and does not involve any human, biometric, or sensitive data. The 3D models are sourced from Objaverse, the environment lighting maps are from public open-source datasets, and the material properties are based on lab-measured spectra of real-world materials. All data sources and usage conform to the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work provides a benchmark dataset for material-aware 3D reconstruction, which may positively contribute to scientific progress in physically grounded 3D vision, digital twin, autonomous driving, and robotics. Since the dataset is semi-synthetic and does not include human-related data, privacy and fairness concerns are minimal. However, like any dataset enabling realistic rendering, there is a potential risk of misuse in deceptive content generation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer:  \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The dataset is semi-synthetic, built from publicly available 3D models, lab-measured material spectra IOR, and open-source environment maps. It does not contain human data, sensitive content, or scraped web data, and poses minimal risk of misuse requiring specific safeguards.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The dataset as a whole is licensed under the CC BY-NC 4.0 DEED. However, individual 3D object shapes within the dataset are subject to different licenses. For more details on each object's specific license, please refer to Objaverse's documentation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We introduce a new semi-synthetic dataset, OpenMaterial, and provide detailed documentation including dataset structure, licensing information, and usage guidelines. The generation code and material-related data will be released alongside the dataset to support reproducibility and responsible use.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve any crowdsourcing or research with human subjects. All data is generated from synthetic or publicly available non-human assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work does not involve human subjects or crowdsourcing and therefore does not require IRB or equivalent ethical approval.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Large language models were not used as part of the core methods, experiments, or data generation in this research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

